DiLA: Enhancing LLM Tool Learning with Differential Logic Layer

Considering the challenges faced by large language models (LLMs) in logical reasoning and planning, prior efforts have sought to augment LLMs with access to external solvers. While progress has been made on simple reasoning problems, solving classical constraint satisfaction problems, such as the Boolean Satisfiability Problem (SAT) and Graph Coloring Problem (GCP), remains difficult for off-the-shelf solvers due to their intricate expressions and exponential search spaces. In this paper, we propose a novel differential logic layer-aided language modeling (DiLA) approach, where logical constraints are integrated into the forward and backward passes of a network layer, to provide another option for LLM tool learning. In DiLA, LLM aims to transform the language description to logic constraints and identify initial solutions of the highest quality, while the differential logic layer focuses on iteratively refining the LLM-prompted solution. Leveraging the logic layer as a bridge, DiLA enhances the logical reasoning ability of LLMs on a range of reasoning problems encoded by Boolean variables, guaranteeing the efficiency and correctness of the solution process. We evaluate the performance of DiLA on two classic reasoning problems and empirically demonstrate its consistent outperformance against existing prompt-based and solver-aided approaches.

==> doc/checklist.tex <==
\section{Reproducibility Checklist}

This paper:
\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes)
    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes)
    \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (yes)
\end{itemize}

Does this paper make theoretical contributions? (yes)

If yes, please complete the list below.
\begin{itemize}
    \item All assumptions and restrictions are stated clearly and formally. (yes)
    \item All novel claims are stated formally (e.g., in theorem statements). (yes)
    \item Proofs of all novel claims are included. (partial)
    \item Proof sketches or intuitions are given for complex and/or novel results. (partial)
    \item Appropriate citations to theoretical tools used are given. (yes)
    \item All theoretical claims are demonstrated empirically to hold. (yes)
    \item All experimental code used to eliminate or disprove claims is included. (no)
\end{itemize}

Does this paper rely on one or more datasets? (yes)

If yes, please complete the list below.
\begin{itemize}
    \item A motivation is given for why the experiments are conducted on the selected datasets (yes)
    \item All novel datasets introduced in this paper are included in a data appendix. (yes)
    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes)
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes)
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes)
    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes)
    \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes)
\end{itemize}

Does this paper include computational experiments? (yes)

If yes, please complete the list below.
\begin{itemize}
    \item Any code required for pre-processing data is included in the appendix. (no).
    \item All source code required for conducting and analyzing the experiments is included in a code appendix. (no)
    \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes)
    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (NA)
    \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes)
    \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes)
    \item This paper states the number of algorithm runs used to compute each reported result. (yes)
    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes)
    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes)
    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes)
\end{itemize}


==> doc/limitation.tex <==
\section{Limitation}

We identify two main limitations of DiLA. First, DiLA relies on translating reasoning problems into logical formats that can be encoded by boolean variables and first-order logic. As a consequence, the model’s applicability is inherently bounded by the expressiveness of the underlying theory, as not all problems can be easily encoded in first-order formulas with boolean vectors. Nevertheless, the wide range of tasks that we can instantiate our DiLA framework on shows its general applicability.

Second, DiLA relies on backbone LLMs to translate natural language problems into symbolic representations. Although this approach has shown promise, it may struggle with logical representations featuring complex grammar structures, such as probabilistic circuit logic. This limitation stems from the challenge of communicating intricate grammatical rules to the language model through a limited number of demonstrations within a constrained context size. To address this, future research could investigate the development of specialized modules to improve the mapping between natural language and symbolic language, for instance, by fine-tuning LLMs with symbolic formulas for specific reasoning tasks.

==> doc/overview.tex <==
\section{Overview}



\begin{figure*}[htbp]
    \centering
    \includegraphics[width = .95\linewidth]{dila}
    \caption{The overall flow of DiLA. Starting from a problem in natural language, in \emph{Step 1}, the LLM parses it into a SAT problem specification which consists of a set of logical formulas. Then in \emph{Step 2}, the backbone LLM tries to output an initial solution based on its language understanding. In \emph{Step 3}, the relaxed variables and extracted constraints are offloaded to a differential logic layer, checking the constraint satisfiability, and updating the solution until all constraints are met. Here, the solid arrow indicates the forward pass, while the dashed arrow represents the backward pass. }
    \label{fig:dila}
\end{figure*}

In this section, we present DiLA, which augments LLM with the ability of logical reasoning by incorporating a differential logic layer. More specifically, DiLA addresses the challenge of using LLMs to tackle canonical reasoning tasks expressed in natural language. These tasks typically involve presenting a set of premises and constraints, prompting questions that necessitate intricate deductive reasoning over the provided inputs, which remains a formidable challenge even for contemporary LLMs~\citep{valmeekam2022large}. 

Notably, the Satisfiability (SAT) problem can serve as a versatile intermediate step for solving a broad range of constraint satisfaction problems, provided they can be expressed using Boolean variables. Specifically, problem instances from NP-complete domains, such as Graph Coloring and Set Cover, can be seamlessly encoded into SAT problem specifications, thereby allowing for efficient solutions via SAT algorithms~\citep{graphcolor, satlayout}. Therefore, we harness SAT encoding as a general bridge to tackle these constraint satisfaction problems in practical settings.

% At a high level, given the natural language description of a collection of facts $\phi$ (such as propositions or constraints) about some variables $V$, the LLM is prompted with a question $Q$ related to these variables.
% The ultimate goal of the reasoning task is to determine an answer to $Q$, which essentially entails identifying the assignment for the variable of interest that satisfies all the input constraints $\phi$.

The general procedure for solving natural language reasoning tasks with DiLA can be conceptualized in three distinct steps: parsing, initialization, and refinement. Given a natural language input that describes both the propositional constraints $\phi$ and the question $Q$, we first parse this input into a SAT specification using LLMs, thereby obtaining a formal description of the constraints and variables. Next, we leverage the LLM's natural language understanding to generate an initial variable assignment. Since this initial solution may only partially satisfy the propositional constraints, DiLA iteratively refines it through a differential logic layer that encodes all of the logical formulas, ultimately yielding a more accurate solution. \Cref{fig:dila} illustrates the overall flow of our proposed DiLA.





%===============

%To make the mathematical derivation smooth, each assignment of all literals is defined as the function $f$ from literals to solution space. From this perspective, SAT is a special case of boolean variables when the solutions space is defined as $\{1, -1\}$. We define a  as the values of a literal subset in V. 


%===================
% \subsection{Towards UNSAT Proving}\label{sec:unsat}


% In general, an UNSAT instance denotes that, over all possible assignments of the literals, there exist at least two clauses that cannot be satisfied simultaneously. Let's consider the CNF formula $\phi$, where $S$ is a subset of variables, and $D$ defines the solution space. In the theory of satisfiability, the following lemma is based on the backdoor counting results~\citep{backdoor},

% \textbf{Lemma~1} Given a CNF formula $\phi$ with $n$ variables, for all subsets $S$ of the $n$ variables with $|S|=i$, perform a standard backtracking search (solely on the variables in $S$) for an assignment that resolves $C$. The search time for finding this assignment is $O\left(p(n)\frac{dn}{B(n)^{1/2}}^{B(n)} \right)$, where $p(n)$ is some polynomial.

% Therefore, based on \textbf{Lemma~1}, we can have a conclusion for UNSAT proving: 

% \textbf{Theorem~1} Considering the structure of the search tree, if every leaf in the search tree concludes with sub-assignments indicating unsatisfiability, the original CNF formula $\phi$ is deemed UNSAT with a probability of 1.


% The proof is evident. Each leaf of the search tree represents a partial assignment for the original formula $\phi$. It is clear that if all partial assignments indicate the existence of two clauses that cannot be satisfied simultaneously, the formula is UNSAT. Returning to the LLM for SAT solving, when the LLM is given a CNF, it can at least provide an assignment that satisfies part of the original clauses. Based on Lemma 1 and Theorem 1, the problem can be refined to the final solution in polynomial time. If, in some iterations, all subproblems are found to be UNSAT, then the original problem is UNSAT. We can further draw the following conclusions, culminating in the complete proof of UNSAT scenarios:

% \textbf{Corollary~1} If all leaves end with the sub-assignments reporting satisfiability, we can always get a minimal unsatisfied assignment by adding constraints in polynomial loops. \label{corollary}

% Now the problem of UNSAT proving involves efficiently finding the unsatisfied subproblem. Here we we illustrate our approach with a simple example. Clearly, $\phi = (x_1) \wedge (\neg x_1) \wedge (\neg x_1 \vee x_2) \wedge (\neg x_2) $ has a MaxSAT solution with three satisfied clauses: $(\neg x_1) \wedge (\neg x_1 \vee x_2) \wedge (\neg x_2)$. Consider $(x_1)$, the clause not included in the MaxSAT solution, it provides useful information. If it is removed from $\phi$, the resulting formula is satisfiable. Therefore, we denote such clauses as $\bar{\phi^\prime}$, where $\phi^\prime$ is the MaxSAT solution of $\phi$. In other words, $\bar{\phi^\prime}$ is a complementary set of $\phi^\prime$.

% This complementary view of $\phi^\prime$ reveals another connection between maximum satisfiability and minimally unsatisfiable cores (MUC). Particularly, a minimally unsatisfiable core is an unsatisfiable subset of the clauses in such that removing any clause from the set makes it satisfiable. In other words, none of the clauses in the core are superfluous, i.e., deleting any singleton clause from MUC will cause it to be satisfiable. Because the presence of any MUC in a formula makes it unsatisfiable, at least one clause from every MUC must be removed to make it satisfiable. That is, given an unsatisfiable formula $\phi$ and a set of clauses $\gamma \subseteq \phi$, $\phi^\prime = \phi \backslash \gamma$ is satisfiable if and only $\gamma$ contains at least one clause from $\bar{\phi^\prime}$. Therefore, $\bar{\phi^\prime}$ must contain at least one clause from minimally unsatisfiable subformulas. As the maximum satisfiable set $\phi^\prime$ can be readily obtained by its SDP relaxation, i.e., \Cref{eq:2}, surely we can leverage its complement $\bar{\phi^\prime}$ to iteratively find unsatisfiable subproblems (see more details in \Cref{sec:unsat_procedure}). 

% We assume that the original SAT problem can always be divided into different groups based on the sparsity of clause matrix $S \in \{1,-1,0 \}^{m \times n}$. We assume that the group number is $k$, and in case there is no cluster among the , it means that $k=1$. Supposing that there exists a partial assignments $a_S: S \longrightarrow D$ such as $\phi$ is satisfiable, S is defined as \textit{backdoor} if $a_S$ can return a satisfying assignments
 






==> setting-acm.tex <==
% =============================================================
%         Setting for ACM 2017 format
%
%   Author      : Bei Yu
%   Last Update : 11/2023
% =============================================================

\settopmatter{printacmref=false}          % no ACM Reference Format
\fancyhead{}                              % no header

% ==== page margin settings
\iffalse
\geometry{twoside=true, head=13pt,
	paperwidth=8.5in, paperheight=11in,
	includeheadfoot, columnsep=2pc,
	top=57pt, bottom=73pt, inner=54pt, outer=54pt,
	marginparwidth=2pc,heightrounded
}%
\fi

\iffalse
% === shrink page num
\usepackage{titlesec}
\titlespacing\section{2pt}{5pt plus 1pt minus 1pt}{0pt plus 1pt minus 1pt}
\titlespacing\subsection{2pt}{5pt plus 1pt minus 1pt}{0pt plus 1pt minus 1pt}
\titlespacing\subsubsection{2pt}{5pt plus 1pt minus 1pt}{2pt plus 1pt minus 1pt}
\fi

\iffalse
\setlength{\textfloatsep}{6pt plus 1pt minus 1pt}          % set space between float and text
\setlength{\floatsep}{8pt plus 1pt minus 1pt}              % set space between two floats
\setlength{\intextsep}{4pt plus 1pt minus 1pt}             % set space between text and float
\setlength{\columnsep}{16pt}                               % set space between columns
% ==== reduce space around equations
\setlength{\belowdisplayskip}{4pt} \setlength{\belowdisplayshortskip}{4pt}
\setlength{\abovedisplayskip}{4pt} \setlength{\abovedisplayshortskip}{4pt}
\fi
%\intextsep             = 0pt plus 1pt minus 7pt           % set space above and below the texts
%\dbltextfloatsep       = 0pt plus 1pt minus 7pt
%\dblfloatsep           = 0pt plus 1pt minus 7pt
%\abovedisplayskip      = 0pt plus 1pt minus 7pt           % set space around equations
%\belowdisplayskip      = 0pt plus 1pt minus 7pt
%\abovedisplayshortskip = 0pt plus 1pt minus 7pt
%\belowdisplayshortskip = 0pt plus 1pt minus 7pt

% ==== Packages
\usepackage{lipsum}
\usepackage{graphicx}
\usepackage{footnote}
\let\Bbbk\relax
\usepackage{amssymb}
\newcommand\bmmax{0}
\newcommand\hmmax{0}
\usepackage{footnote}
\usepackage{amsmath}
\usepackage{mathtools}
\usepackage{mathrsfs}                                      % mathscr command
\usepackage{siunitx} \sisetup{detect-all}
\usepackage{comment}
\usepackage{wrapfig} 
% \usepackage[subrefformat=parens,labelformat=parens]{subfig}
\captionsetup[subfigure]{labelformat=simple}               % avoid "double brackets" in sub-figure caption
% \renewcommand\thesubfigure{(\alph{subfigure})}             % "Fig.~1b"-->"Fig.1(b)"
\usepackage{bm,bbm}
\usepackage{multirow}
\usepackage{makecell}
\usepackage{threeparttable,booktabs}
\usepackage{blkarray}
\usepackage{tikz}
\usetikzlibrary{positioning,calc,fit,decorations.pathmorphing,shapes.geometric,shapes.gates.logic.US,calc}
\usepackage{tikz-3dplot}
\usepackage{balance}
\usepackage{courier}                                       % courier font, used in \texttt
\usepackage{pifont}                                        % ding commend
\usepackage{cleveref}                                      % smart citation
%\Crefformat{figure}{Fig.~#2#1#3}                           % "Fig.", instead of "Figure"
%\Crefname{subfigure}{Fig.}{Figs.}
%\Crefname{figure}{Fig.}{Figs.}
\usepackage[mathcal]{eucal}
\iffalse
%\usepackage[noend]{algorithm2e}
\usepackage[]{algpseudocode}                               % algorithm package
% \usepackage[noend]{algpseudocode}
\algrenewcommand\textproc{\texttt}
\makeatletter\let\float@addtolists\relax\makeatother
\usepackage{algorithm}
\renewcommand{\algorithmicrequire}{\textbf{Input:} }       % Use Input in the format of Algorithm
\renewcommand{\algorithmicensure} {\textbf{Output:}}       % Use Output in the format of Algorithm
\algblockdefx[pardo]{pardo}{endpardo}%
   [1]{\textbf{For} #1 \textbf{do in parallel}}%
   {\textbf{Endfor}}
\fi
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{filecontents}                                  % support to pgfplots
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\usepackage{pgf-pie}
\usepgfplotslibrary{groupplots}
\pgfplotsset{compat=newest}
\usepackage[figuresright]{rotating}
\usepackage{xcolor,colortbl}                               % \rowcolor
%\usepackage[cache=false,outputdir=./]{minted}             % code highlight, w. "--shell-escape" in pdflatex
\iffalse
\IfFileExists{minted_configuration.tex}{\input{minted_configuration.tex}}{\usepackage[outputdir=../]{minted}}
\setminted{escapeinside=@@, fontsize=\tiny, numbersep=8pt, breaklines=true, linenos=false}
\fi
\usepackage[inline]{enumitem}                              % inline enumerate
\setlist{leftmargin=5.08mm}

% ==== Local new commands
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\etal}{\textit{et al.}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\tool}[1]{$\mathsf{#1}$}
\newcommand{\m}[1]{\boldsymbol{#1}}
\newcommand{\abs}[1]{\ensuremath{\left\lvert #1\right\rvert}}
\newcommand{\tensor}[1]{\mathcal{#1}}      % define tensor command
\renewcommand{\vec}[1]{\boldsymbol{#1}}
% \renewcommand{\vec}[1]{\mathbf{#1}}
\newcommand{\todo}[1]{\textcolor{red}{[TODO: #1]}}
\newcommand{\revise}[1]{\textcolor{blue}{#1}}
\newcommand{\minisection}[1]{\vspace{.08in}\noindent{\textbf{#1}}.}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}

\theoremstyle{plain}
\newtheorem{mytheorem}{\textbf{Theorem}}
\newtheorem{mylemma}{\textbf{Lemma}}
\newtheorem{mycorollary}{Corollary}
\newtheorem{myclaim}{\textbf{Claim}}
\newtheorem{myproperty}{\textbf{Property}}
\newtheorem{myassumption}{\textbf{Assumption}}

\theoremstyle{definition}
\newtheorem{mydefinition}{\textbf{Definition}}
\newtheorem{myproblem}{\textbf{Problem}}

\newcommand{\tabincell}[2]{
    \begin{tabular}{@{}#1@{}}#2\end{tabular}
}

% ==== spacing control on caption
\usepackage[skip=1pt]{caption}            % set space between figure and caption
\setlength{\belowcaptionskip}{-1.0mm}
\captionsetup[table]{aboveskip=5pt}       % reduce space around table caption
\captionsetup[table]{belowskip=2pt}

% ==== local color definitions
\definecolor{CUHKorange}{RGB}{244,106,18} %F47012
\definecolor{CUHKblue}{RGB}{0,111,190}    %006FBE
\definecolor{CUHKgreen}{RGB}{0,127,128}   %007F80
\definecolor{CUHKred}{RGB}{228,46,36}     %E42E24
\definecolor{CUHKyellow}{RGB}{198,148,34} %C69422
\definecolor{CUHKdark}{RGB}{114,44,114}   %722C72
\definecolor{CUHKmiddle}{RGB}{144,44,144} %902C90

% === beamer style block
\usepackage{tcolorbox}
\tcbuselibrary{skins,breakable}
\newenvironment{myblock}[1]{%
    \tcolorbox[beamer,%
    noparskip,breakable,
    colback=white,colframe=CUHKmiddle,%
    colbacklower=white,%
    title=#1]}%
    {\endtcolorbox}


